Stabilized RANS simulation of surf zone kinematics and boundary layer processes beneath large-scale plunging waves over a breaker bar

This paper presents numerical simulations of a bichromatic wave group propagating and breaking over a fixed breaker bar. The simulations are performed using a newly stabilized Reynolds-averaged Navier Stokes (RANS) two-equation turbulence closure, which solves the longstanding problem of over-production of turbulence beneath surface waves in the nearly potential flow region prior to breaking. This model has previously been tested on small-scale spilling breaking regular waves, whereas in this work focus is on full (rather than model) scale application, wave groups (rather than regular waves) and plunging (rather than spilling) breakers. Additionally this paper has novel emphasis on bottom boundary layer dynamics which are very important for cross-shore sediment transport predictions. The model is validated by comparing with results from a previous experimental campaign. The model is shown to predict the surface elevations, velocities and turbulence well in the shoaling and outer surf-zone, avoiding turbulence over-production and incorrect undertow structure typical of standard turbulence closures. Comparison with detailed boundary layer measurements in the shoaling position reveals that the model is able to accurately capture the temporal dynamics of the entire wave boundary layer, including evolution of the boundary layer thickness, velocity overshoot and phase-shifts. Comparison in the surf zone additionally reveals that the model is able to accurately capture the transport of breaking-induced turbulence into the wave boundary layer. The performance of the model indicates that it can be used directly in the simulation of cross-shore sediment transport and morphology and also be used to study important hydrodynamic processes, which can help improve the predictive skill of morphodynamic profile models applied in coastal engineering.

==> makefile <==
# Makefile for LATEX compiling

# Base filename of LATEX file (without .tex)
FNAME=Fuhrmanetal

all:
	latex $(FNAME)
	bibtex $(FNAME)
	latex $(FNAME)
	latex $(FNAME)

bib: 	
	latex $(FNAME)
	bibtex $(FNAME)

ps:
	latex $(FNAME)
	latex $(FNAME)
	dvips $(FNAME).dvi -Ppdf -G0 -o $(FNAME).ps
	gv $(FNAME).ps

dvi:
	latex $(FNAME)
	latex $(FNAME)
	xdvi $(FNAME)

pdf:

	latex $(FNAME)
	latex $(FNAME)
	dvips $(FNAME).dvi -Ppdf -G0 -o $(FNAME).ps

	ps2pdf -sPAPERSIZE=a4 \
	-dMaxSubsetPct=100 -dCompatibilityLevel=1.2 \
	-dSubsetFonts=true -dEmbedAllFonts=true \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dModoImageFilter=/FlateEncode \
	$(FNAME).ps $(FNAME).pdf
	acroread $(FNAME).pdf

clean:
#	rm -f *.pdf
	rm -f *.ps
	rm -f *.dvi
	rm -f *.log
	rm -f *.bbl
	rm -f *.blg
	rm -f *.aux
	rm -f *.spl
	rm -f *~
